Proofs of Proof-of-Stake with Sublinear Complexity

Popular Ethereum wallets (like MetaMask) entrust centralized infrastructure providers (e.g., Infura) to run the consensus client logic on their behalf. As a result, these wallets are light-weight and high-performant, but come with security risks. A malicious provider can mislead the wallet by faking payments and balances, or censoring transactions. On the other hand, light clients, which are not in popular use today, allow decentralization, but are concretely inefficient, often with asymptotically linear bootstrapping complexity. This poses a dilemma between decentralization and performance. We design, implement, and evaluate a new proof-of-stake (PoS) superlight client with concretely efficient and asymptotically logarithmic bootstrapping complexity. Our proofs of proof-of-stake (PoPoS) take the form of a Merkle tree of PoS epochs. The verifier enrolls the provers in a bisection game, in which honest provers are destined to win once an adversarial Merkle tree is challenged at sufficient depth. We provide an implementation for mainnet Ethereum: compared to the state-of-the-art light client construction of Ethereum, our client improves time-to-completion by 9x, communication by 180x, and energy usage by 30x (when bootstrapping after 10 years of consensus execution). As an important additional application, our construction can be used to realize trustless cross-chain bridges, in which the superlight client runs within a smart contract and takes the role of an on-chain verifier. We prove our construction is secure and show how to employ it for other PoS systems such as Cardano (with fully adaptive adversary), Algorand, and Snow White.

==> 10_acknowledgements.tex <==
\section*{Acknowledgment}

The authors thank Kostis Karantias for the helpful discussions on bisection games,
and Daniel Marin for reading early versions of this paper and providing suggestions.
%
%
The work of JN
was conducted in part
while at Paradigm.
%
%
JN is supported by the Protocol Labs PhD Fellowship.
%
ENT is supported by the Stanford Center for Blockchain Research.
The work of DZ was supported in part by funding from Harmony.


==> algorithms/alg.make.merkle.tree.tex <==
\begin{algorithm}[tb]
    \caption{Creates a Merkle tree using the given data.}
    \label{alg.make.merkle.tree}
    \begin{algorithmic}[1]\small
        \Function{\sc MakeMT}{\rm data}
            \If{$|\textrm{data}|=1$}
                \State\Return $\textsc{Tree}(\textrm{root}$: $H(\textrm{data}[0]), \textrm{data}$: $\textrm{data}[0])$
            \EndIf
            \State\Let{\rm mid}{\lfloor\frac{|\textrm{data}|}{2}\rfloor}
            \State $\textrm{tree} \gets \textsc{Tree}($
                \State \quad$\textrm{left}$: $\textsc{MakeMT}(\textrm{data}[{:}\textrm{mid}]),$
                \State \quad$\textrm{right}$: $\textsc{MakeMT}(\textrm{data}[\textrm{mid}{:}])$
                \State $)$
            \State\Let{\textrm{tree.root}}{H(\textrm{tree.left.root}\concat\textrm{tree.right.root})}
            \State\Return\textrm{tree}
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> algorithms/alg.make.mmr.tex <==
\begin{algorithm}[tb]
    \caption{Creates a Merkle Mountain Range using the given data for the leaves.
        Here, \textsc{MakeMT} takes data of size $2^q$ and constructs a Merkle Tree out of it.}
    \label{alg.make.mmr}
    \begin{algorithmic}[1]\small
        \Function{\sc MakeMMR}{\rm data}
            \If{$|\textrm{data}|=0$}
                \State\Return $[\,]$
            \EndIf
            \State\Let{\rm bound}{2^{\lfloor\log|\textrm{data}|\rfloor}}
            \State\Let{\rm head}{\textsc{MakeMT}(\textrm{data}[{:}\textrm{bound}]})
            \State\Let{\rm tail}{\textsc{MakeMMR}(\textrm{data}[\textrm{bound}{:}]})
            \State\Return $(\textrm{head}{:}\textrm{tail})$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> bibliography/bibliography.tex <==
\bibliography{%
bibliography/humanities,%
bibliography/math,%
bibliography/crypto,%
bibliography/cs,%
bibliography/blockchains,%
bibliography/interoperability,%
bibliography/implementation,%
bibliography/ours,%
bibliography/thesis%
}
\ifuniversity
\addcontentsline{toc}{chapter}{REFERENCES}
\fi


==> figures/plots/TMP_experiment-1/figure.tex <==
\pgfplotsset{
    myexp1plt/.style={
            nodes near coords,
            point meta=explicit symbolic,
            visualization depends on={value \thisrow{style}\as\mystyle},
            every node near coord/.append style={font=\footnotesize,\mystyle},
        },
}

\begin{figure}[tb]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
                mysimpleplot,
                xlabel={Total communication [Mbytes]},
                xmin=0, xmax=200,
                %
                ymin=0, ymax=200,
                width=0.5\linewidth,
                height=0.4\linewidth,
                %
                legend columns=8,
                legend style={
                        at={(0.5,1)},
                        yshift=0.3em,
                        anchor=south,
                        draw=none,
                        /tikz/every even column/.append style={
                                column sep=0.3em
                            },
                        cells={
                                align=left
                            },
                        xshift=-3.25cm,
                    },
            ]


            \addlegendimage{myClientLC1};
            \addlegendentry{\expLClegend};
            \addlegendimage{myClientOLC1};
            \addlegendentry{\expOLClegend};
            \addlegendimage{myClientSLC1};
            \addlegendentry{\expSLClegend};

            \addlegendimage{myClientLC2,mark=none,gray};
            \addlegendentry{5\,y};
            \addlegendimage{myClientLC1,mark=none,gray};
            \addlegendentry{10\,y};
            \addlegendimage{myClientLC3,mark=none,gray};
            \addlegendentry{15\,y};
            \addlegendimage{myClientLC4,mark=none,gray};
            \addlegendentry{20\,y};
            \addlegendimage{myClientLC5,mark=none,gray};
            \addlegendentry{30\,y};



            \addplot+ [
                myexp1plt,
                myClientLC2,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/light-T1850.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientLC1,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/light-T3650.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientLC3,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/light-T5475.txt};
            %



            \addplot+ [
                myexp1plt,
                myClientOLC2,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/optimisticlight-T3650.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientOLC4,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/optimisticlight-T7300.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientOLC5,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/optimisticlight-T10950.txt};
            %



            \addplot+ [
                myexp1plt,
                myClientSLC2,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/superlight-T3650.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientSLC4,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/superlight-T7300.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientSLC5,
                no marks,
                forget plot,
            ] table [
                    x=bandwidth,
                    y=delay,
                    %
                ] {figures/plots/experiment-1/superlight-T10950.txt};
            %



            \coordinate (boxA1) at ([xshift=1.5pt,yshift=1.5pt] 5,60);
            \coordinate (boxB1) at ([xshift=-1.5pt,yshift=-1.5pt] 0,0);

        \end{axis}
        %
        \draw [ultra thick, densely dotted] (boxA1) rectangle (boxB1);
        %
        %
        %
        %
        %
        %
        \begin{axis}[
            mysimpleplot,
            xlabel={Total communication [Mbytes]},
            xmin=0, xmax=5,
            ylabel={Time-to-completion [seconds]},
            ymin=0, ymax=60,
            width=0.5\linewidth,
            height=0.4\linewidth,
            %
            %
            %
            xshift=-6.5cm,
            %
            %
            %
            %
            ]

            \addplot+ [
                myexp1plt,
                myClientOLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/optimisticlight-T3650.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientOLC4,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/optimisticlight-T7300.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientOLC5,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/optimisticlight-T10950.txt};
            %



            \addplot+ [
                myexp1plt,
                myClientSLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/superlight-T3650.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientSLC4,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/superlight-T7300.txt};
            %

            \addplot+ [
                myexp1plt,
                myClientSLC5,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-1/superlight-T10950.txt};
            %


            \legend{};


            \coordinate (boxA2) at (5,60);
            \coordinate (boxB2) at (5,0);

        \end{axis}
        %
        \draw [ultra thick, densely dotted, opacity=0.3] (boxA1) -- (boxA2);
        \draw [ultra thick, densely dotted, opacity=0.3] (boxB1) -- (boxB2);
        %
        %
    \end{tikzpicture}%
    %
    \caption{%
        Time-to-completion and total communication
        (averaged over $5$ trials)
        incurred
        by different light clients
        %
        for varying internal parameters (marker labels; \expLClegend/\expOLClegend: batch size $b$,
        \expSLClegend: Merkle tree degree $d$)
        and varying execution horizon.
        %
        Pareto-optimal tradeoffs are
        %
        at `tip' of resulting
        `L-shape':
        for $10$ years execution,
        %
        at
        $b\approx200$, $b\approx500$, and $d\approx100$,
        respectively.
        %
        \expOLClegend and \expSLClegend vastly outperform
        \expLClegend,
        %
        \eg,
        for $10$ years execution:
        $9\times$ in time-to-completion,
        $180\times$ in bandwidth.
        In this setting, \expSLClegend has similar time-to-completion as \expOLClegend,
        and $3\times$ lower communication.
        %
        %
        %
        %
        %
        %
        %
        %
        %
        %
        %
        %
        %
    }
    \label{fig:experiment-experiment-1}
\end{figure}


==> figures/plots/experiment-0/figure.tex <==
%
%
%
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            mysimpleplot,
            xlabel={Total communication [Mbytes]},
            xmin=0, xmax=10,
            ylabel={Time-to-completion [seconds]},
            ymin=0, ymax=60,
            %
            height=0.6\linewidth,
            ]

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientOLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-0/optimisticlight-T10950.txt};
            \addlegendentry{Optimistic LC};

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientSLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-0/superlight-T10950.txt};
            \addlegendentry{Super-LC};

        \end{axis}
    \end{tikzpicture}%
    \vspace{-0.75em}%
    \caption{%
        ...%
        %
        %
        %
        %
        %
    }
    \label{fig:experiment-experiment-0}
\end{figure}


==> figures/plots/experiment-4/figure.tex <==
%
%
%
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            mysimpleplot,
            xlabel={Total communication [Mbytes]},
            xmin=0, xmax=5,
            ylabel={Time-to-completion [seconds]},
            ymin=0, ymax=50,
            %
            height=0.6\linewidth,
            %
            legend columns=2,
            ]

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientOLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-4/optimisticlight-T1825.txt};
            \addlegendentry{Optimistic LC (5y)};

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientOLC2,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-4/optimisticlight-T3650.txt};
            \addlegendentry{Optimistic LC (10y)};

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientSLC1,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-4/superlight-T1825.txt};
            \addlegendentry{Super-LC (5y)};

            \addplot+ [
                nodes near coords,
                point meta=explicit symbolic,
                visualization depends on={value \thisrow{style}\as\mystyle},
                every node near coord/.append style={font=\footnotesize,\mystyle},
                myClientSLC2,
            ] table [
                    x=bandwidth,
                    y=delay,
                    meta=label,
                ] {figures/plots/experiment-4/superlight-T3650.txt};
            \addlegendentry{Super-LC (10y)};

        \end{axis}
    \end{tikzpicture}%
    \vspace{-0.75em}%
    \caption{%
        ...%
        %
        %
        %
        %
        %
    }
    \label{fig:experiment-experiment-0}
\end{figure}


==> macros.tex <==
\def\chain{\mathcal{C}}
\newcommand{\concat}{\,\|\,}

\newcommand{\true}{\ensuremath{\mathsf{true}}}
\newcommand{\false}{\ensuremath{\mathsf{false}}}

\def\Let#1#2{$#1\gets#2$}
\newcommand{\CommentLine}[1]{%
    \State \(\triangleright\) \textit{#1}%
}
\newcommand{\Break}{\State\textsf{break}}
\newcommand{\Continue}{\State\textsf{continue}}

\newcommand{\tx}{\ensuremath{\mathsf{tx}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Tconf}{\ensuremath{T_\mathrm{conf}}}
\newcommand{\Twait}{\ensuremath{T_\mathrm{wait}}}

%


\usepackage{xspace}
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\cfinalized}{client-finalized\xspace}
\newcommand{\cfinalize}{client-finalize\xspace}
\newcommand{\cfinalizes}{client-finalizes\xspace}

%
\renewcommand{\st}{\ensuremath{\mathsf{st}}}
\newcommand{\stc}{\ensuremath{\left<\st\right>}}
\newcommand{\transition}{\delta}

\newcommand{\mroot}{\ensuremath{\left<\mathcal{T}\right>}}
\newcommand{\negl}{\mathrm{negl}}
\newcommand{\ledger}{\ensuremath{\mathbb{L}}}
\newcommand{\genesisstate}{\st_0}

\newcommand{\client}{\mathcal{V}}

\newcommand{\Ourprotocol}{Our superlight client\xspace}
\newcommand{\ourprotocol}{our superlight client\xspace}
\newcommand{\Optclient}{Optimistic light client\xspace}
\newcommand{\optclient}{optimistic light client\xspace}
\newcommand{\OptClient}{Optimistic Light Client\xspace}

\newcommand{\hon}[1]{{\color{OliveGreen} #1}}
\newcommand{\adv}[1]{{\color{red} #1}}
\newcommand{\prover}[1]{{\color{blue} #1}}
\newcommand{\verifier}[1]{{\color{orange} #1}}

\newcommand{\expLClegend}{TLC\xspace}
\newcommand{\expLC}{traditional light client\xspace}
\newcommand{\ExpLC}{Traditional light client\xspace}
\newcommand{\expOLClegend}{OLC\xspace}
\newcommand{\expOLC}{optimistic light client\xspace}
\newcommand{\ExpOLC}{Optimistic light client\xspace}
\newcommand{\expSLClegend}{SLC\xspace}
\newcommand{\expSLC}{superlight client\xspace}
\newcommand{\ExpSLC}{Superlight client\xspace}

%
%
%
%
\newcommand{\myparagraph}[1]{%
    \subparagraph*{#1}%
}

